Deterministic Dynamic Matching In Worst-Case Update Time

We present deterministic algorithms for maintaining a $(3/2 + \epsilon)$ and $(2 + \epsilon)$-approximate maximum matching in a fully dynamic graph with worst-case update times $\hat{O}(\sqrt{n})$ and $\tilde{O}(1)$ respectively. The fastest known deterministic worst-case update time algorithms for achieving approximation ratio $(2 - \delta)$ (for any $\delta > 0$) and $(2 + \epsilon)$ were both shown by Roghani et al. [2021] with update times $O(n^{3/4})$ and $O_\epsilon(\sqrt{n})$ respectively. We close the gap between worst-case and amortized algorithms for the two approximation ratios as the best deterministic amortized update times for the problem are $O_\epsilon(\sqrt{n})$ and $\tilde{O}(1)$ which were shown in Bernstein and Stein [SODA'2021] and Bhattacharya and Kiss [ICALP'2021] respectively. In order to achieve both results we explicitly state a method implicitly used in Nanongkai and Saranurak [STOC'2017] and Bernstein et al. [arXiv'2020] which allows to transform dynamic algorithms capable of processing the input in batches to a dynamic algorithms with worst-case update time. \textbf{Independent Work:} Independently and concurrently to our work Grandoni et al. [arXiv'2021] has presented a fully dynamic algorithm for maintaining a $(3/2 + \epsilon)$-approximate maximum matching with deterministic worst-case update time $O_\epsilon(\sqrt{n})$.

==> temp.tex <==
\begin{lemma}

\label{lm:vertexsparsification:adaptive}

Assume there is a dynamic algorithm $Alg$ which maintains an $\alpha = O(1)$ approximate matching in graph $G = (V,E)$ with running time $O(T(n,m))$ provided $\mu(G) \geq \epsilon \cdot |V|$ at all times. Then there is a fully dynamic algorithm $Alg'$ which maintains an $\alpha+\epsilon$ approximate matching for arbitrary graphs in time $O(T(n,m) \cdot \frac{\log^4(n)}{\epsilon^8})$. If the running time of $Alg$ is worst-case (amortized) so will be the running time of $Alg'$. If $Alg$ is robust against adaptive (oblivious) adversaries so will be $Alg'$.

\end{lemma}

\begin{proof}

We will show that Algorithm~\ref{alg:dynamic:matchingsizereduction:adaptive} does what the lemma asks for. First let's argue about the correctness ratio of $Alg'$.

\medskip

At some point during the run of $Alg'$ algorithm $MMSize \leq \mu(G) \leq MMSize \cdot (1 + \epsilon)$. Let's call $MMSize$ at this point as $\mu_\epsilon(G)$ and fix a matching of size $\mu_\epsilon(G)$ in $G$ called $M^*$. There are $\binom{n}{2 \cdot \mu_\epsilon(G)} \leq n^{2 \cdot \mu_\epsilon(G)} = e^{2 \ln(n) \cdot \mu_\epsilon(G)}$ ways the endpoints of $M^*$ could have been selected.

\medskip

Fix a specific definition of vertex subsets $V_{i,j}$. Let $X_i$ stand for the number of vertices set $\V_{i,j}^k$ contains after sampling. Observe that $X_i$ are uniformly distributed and negatively correlated binomial $B(2\cdot \mu_\epsilon(G), \epsilon/\mu_\epsilon(G))$ random variables. Define $Y = \sum X_i$ (for $i \in [\ceil{\frac{MMSize}{\epsilon}}]$). We can apply a Chernoff bound to receive that:

$$P(Y \leq (1 - \epsilon) \cdot E[Y]) \leq e^{-\frac{\epsilon^2 \cdot E[Y]}{2}} = \leq e^{\epsilon^2 \cdot \mu_\epsilon(G)}$$

If $Y\geq(1 - \epsilon)\cdot E[Y] = (1 - \epsilon)\cdot 2 \cdot \mu_\epsilon(G)$ then there can be at most $4 \cdot \epsilon \cdot \mu_\epsilon(G)$ vertices of $M^*$ will be sharing sets $\V_{i,j}^k$ with other vertices hence at least $(1 - 8 \cdot \epsilon) \cdot |M^*|$ edges will have both their endpoints in unique sets. This means $E_{i,j}$ will not contain a matching of size $(1 - 8 \cdot \epsilon) \mu_\epsilon(G)$ with at most $e^{- \mu_\epsilon(G) \cdot \epsilon^2}$. Therefore, none of $E_{i,j} | j \in \frac{4 \ln(n)}{\epsilon^2}$ contains such a matching with probability at most $e^{- 4 \cdot \ln(n) \cdot \mu(G)}$. Summing over all possible selections of the endpoints of $M^*$ we get that at least one $G_{i,j}$ will contain a matching of size $\mu_\epsilon(G) \cdot (1 - 8 \cdot \epsilon)$ with probability $1 - e^{ - 2 \cdot \ln(n) \mu(G)}$ for any graph. 

\medskip

Therefore, one of the $M_{i,j}'$ is at least of size $\mu_\epsilon(G) \frac{1 - 8 \cdot \epsilon}{1 + \alpha} \leq \mu(G)/(10 \epsilon + \alpha)$ for small values of $\alpha$. The algorithm of Gupta and Peng will maintain a matching of size $\frac{\mu(G)}{20 \epsilon + \alpha}$ in the union of all $M_{i,j}'$-s.

\medskip

All sampling and concatenation operations can be done in pre-processing and in linear time. Maintaining each $M_{i,j}'$ in $G$ based on $M_{i,j}$ will take constant time for each change in $M_{i,j}$-s. Similarly, maintaining sparsified the sparsified sub-graphs will also take constant time each. Maintaining $M_{i,j}$ in all $G_{i,j}$ will take time $O(T(n,m) \cdot \frac{\log^2(n)}{\epsilon^3})$ which also serves a recourse bound of $E'$. Max degree of $E'$ is in $O(\frac{\log^2(n)}{\epsilon^3}$ therefore the algorithm of Gupta and Peng will run in $O(\frac{\log^3(n)}{\epsilon^5})$ update time per update to $E'$. This implies that the total update time is $O(\frac{\log^4(n)}{\epsilon^8} \cdot T(n,m))$.


\end{proof}

\begin{corollary}

\label{cor:vertexsparsification:deterministic}

The result of Lemma~\ref{lm:vertexsparsification:adaptive} can be achieved deterministically provided pre-processing takes exponential time.

\end{corollary}

\begin{proof}

Instead of randomly sparsifying the vertex set we may consider every possible random choice we could take and find one which suffices. By the statement of the lemma such a choice must exist.

\end{proof}

\subsection{Deterministic Vertex Set Spasrsification Deterministically Using Expanders}

As Lemma~\ref{lm:vertexsparsification:adaptive} implies for any graph size $n$ there is a way to deterministically sparsify the vertex set. However, finding vertex subsets $V_{i,j}$ seems to be difficult without using randomization. If we are willing to incur a super poly-logarithmic blowup in running time deterministic choices of $V_{i,j}$ can be constructed. The following is a direct result from REFERENCE





\begin{lemma}

\label{lm:support:expander}

REFERENCE: There is a deterministic algorithm which for large enough values of $n$ and $\epsilon \geq 1/poly(\log(n))$ in $poly(n)$ time constructs a $(k, \epsilon)$-expander with $|L| = n$ such that $d = n^{o(1)}$, $|R| = O(\frac{k \cdot d}{poly(\epsilon})))$.

\end{lemma}

\begin{algorithm}[H]
	\SetKwInput{KwInput}{Input}                
	\SetKwInput{KwOutput}{Output}              
	\DontPrintSemicolon
	\label{alg:dynamic:matchingsizereduction:deterministic}
	\caption{Deterministic Vertex Sparsification}
	
	\KwInput{$G = (V,E), Alg$}
	\KwOutput{$\alpha + O(\epsilon)$ matching in $G$}
	$Expander(n,d,k,\epsilon) \leftarrow \text{Deterministic expander construction algorithm of Lemma~\ref{lm:support:expander}}$ \;
	$MMSize \leftarrow 1$ \;
	$i \leftarrow 1$ \;
	$d \leftarrow n^{o(1)}$ \;
    \While{$MMSize \leq n \cdot epsilon$}
    {
        $i \leftarrow i + 1$ \;
        $MMSize \leftarrow MMSize \cdot (1 + \epsilon)$ \;
        $G_{Exp} = ((V,R), E') \leftarrow Expander(n,d,MMSize \cdot 2,\epsilon)$ \;
        \For{$j \in d$}
        {
            Define $|R|$ different sets $V^{v}_{i,j} = \{ v' \in V : N_{E'}(v')_j \}$ for each $v \in R$ \;
            Define $V_{i,j}$ to be a graph with vertices corresponding to non-empty sets $V^v_{i,j} : v \in R$ \;
            Define $E_{i,j}$ as edge concatenated set of vertex sets $V^v_{i,j} : v \in R$ \;
            Generate and maintain sparsified graph $G_{i,j} = (V_{i,j}, E_{i,j})$ \;
            Maintain matching $M_{i,j}$ in $G_{i,j}$ with $Alg$ \;
            Maintain $M_{i,j}$ in $G$ as $M_{i,j}'$\;
        }
    }
    Maintain $M'$ in $G$ with $Alg$ \;
    $E' \leftarrow \underset{i,j}{\cup} M_{i,j}' \cup M'$ \;
    Use Algorithm~\ref{alg:guptapeng} to maintain a $1+ \epsilon$-approximate matching in $(V,E')$ \;
    
\end{algorithm}

\begin{lemma}

\label{lm:vertexsparsification:deterministic}

Assume there is a dynamic algorithm $Alg$ which maintains an $\alpha = O(1)$ approximate matching in graph $G = (V,E)$ with running time $O(T(n,m))$ provided $\mu(G) \geq \epsilon \cdot |V|$ at all times. Then there is a dynamic algorithm $Alg'$ which maintains an $\alpha+\epsilon$ approximate matching for arbitrary graphs in time $O(T(n,m) \cdot n^{o(1)})$. If the running time of $Alg$ is worst-case (amortized) so will be the running time of $Alg'$. If $Alg$ is deterministic then so is $Alg'$.

\end{lemma}

\begin{proof}

We will show that for some $i,j$ it must hold that $\mu(G_{i,j}) \geq (1 - O(\epsilon)) \cdot \mu(G)$ or $\mu(G) \geq n \cdot \epsilon$. Given the first case, $|M_{i,j}| \cdot \alpha \geq (1 - O(\epsilon)) \mu(G)$. Given the second case $M' \cdot \alpha \geq \mu(G)$. 
Since $E' \supset M'_{i,j} \cup M'$ this implies that the algorithm returns an 
$\frac{\alpha}{1 - O(\epsilon)} = \alpha + O(\epsilon)$ approximate matching (given low enough $\epsilon$ and as $\alpha = O(1)$). 

\medskip

Let $i$ be such that during the $i$-th iteration of the outer while loop $MMSize \leq \mu(G) \leq MMSize \cdot (1 + \epsilon)$ (such an $i$ must exist or $\mu(G) \geq n/\epsilon$). Fix a maximum matching in $G$ called $M^*$. Let $V^j_{M^*}$ correspond to it's endpoints in graphs $G_{i,j} : j \in [d]$. By the definition of $(k, \epsilon)$-expanders we know that $\sum_j |V^j_{M^*}| \geq (1 - \epsilon) \cdot 2 \cdot \mu(G) \cdot d$. Therefore, for some $j$ it must hold that $|V^j_{M^*}| \geq \mu(G) \cdot 2 \cdot (1 - \epsilon)$. This means that at least $\mu \cdot (1 - 2 \cdot \epsilon)$ edges of $M^*$ will satisfy that both of their endpoints are concatenated into unique vertices in $V_{i,j}$ with respect to $V^j_{M^*}$. Therefore, $\mu(G_{i,j}) \geq \mu(G) \cdot (1 - O(\epsilon))$.

\medskip

The expander graphs will be generated once in $O(poly(n))$ time. As $i \leq O(\frac{\log (n)}{\epsilon})$ and $j \leq O(n^{o(1)}$ the algorithm will maintain $O(n^{o(1)})$ vertex sparsified sub-graphs, and $\alpha$ approximate matchings within. This will take update time $T(n,m) \cdot \frac{n^{o(1)}}{poly(\epsilon)})$ (as the $n^{o(1)}$ term subsumes the $poly(\log(n))$ terms). The total recourse of $E'$ is bounded by the same amount and a matching is maintained in it in time proportional to it's maximum degree of $O(n^{o(1)}/poly(\epsilon))$. Therefore, the total update time is bounded by $O(T(n,m) \cdot \frac{n^{o(1)}}{poly(\epsilon)})$.

\end{proof}

\begin{algorithm}[H]
	\SetKwInput{KwInput}{Input}                
	\SetKwInput{KwOutput}{Output}              
	\DontPrintSemicolon
	\label{alg:dynamic:matchingsizereduction:adaptive}
	\caption{Vertex Sparsification Against Adaptive Adversaries}
	
	\KwInput{$G = (V,E), Alg$}
	\KwOutput{$\alpha + O(\epsilon)$ matching in $G$}
	$MMSize \leftarrow 1$ \;
	$i \leftarrow 1$ \;
    \While{$MMSize \leq n \cdot \epsilon$}
    {
        $i \leftarrow i + 1$ \;
        $MMSize \leftarrow MMSize \cdot (1 + \epsilon)$ \;
        \For{$j \in \frac{4 \cdot \ln(n)}{\epsilon^2}$}
        {
            Define $\ceil{\frac{MMSize}{\epsilon}}$ different sets $V_{i,j} = \{\V_{i,j}^k : k \in [\ceil{\frac{MMSize}{\epsilon}}]$\} \;
            Uniformly at random assign each vertex $v \in V$ to sets in $V_{i,j}$ \;
            Define $E_{i,j}$ as edge concatenated set of $V_{i,j}$ \;
            Generate and maintain sparsified graph $G_{i,j} = (V_{i,j}^k, E_{i,j}^k)$ \;
            Maintain matching $M_{i,j}$ in $G_{i,j}$ with $Alg$ \;
            Maintain $M_{i,j}$ in $G$ as $M_{i,j}'$\;
        }
    }
    Maintain $M'$ in $G$ using $Alg$ \;
    $E' \leftarrow \underset{i,j}{\cup} M_{i,j}' \cup M'$ \;
    Use Algorithm~\ref{alg:guptapeng} to maintain a $1+ \epsilon$-approximate matching in $(V,E')$ \;
    
\end{algorithm}


